opML: Optimistic Machine Learning on Blockchain

The integration of machine learning with blockchain technology has witnessed increasing interest, driven by the vision of decentralized, secure, and transparent AI services. In this context, we introduce opML (Optimistic Machine Learning on chain), an innovative approach that empowers blockchain systems to conduct AI model inference. opML lies a interactive fraud proof protocol, reminiscent of the optimistic rollup systems. This mechanism ensures decentralized and verifiable consensus for ML services, enhancing trust and transparency. Unlike zkML (Zero-Knowledge Machine Learning), opML offers cost-efficient and highly efficient ML services, with minimal participation requirements. Remarkably, opML enables the execution of extensive language models, such as 7B-LLaMA, on standard PCs without GPUs, significantly expanding accessibility. By combining the capabilities of blockchain and AI through opML, we embark on a transformative journey toward accessible, secure, and efficient on-chain machine learning.

==> layer2.tex <==
\section{Ls-a: AI Optimistic Rollup Layer 2 Blockchain with opML}\label{sec:l2}

opML and optimistic rollup (opRollup) both employ a similar fraud-proof system, making it feasible to integrate opML into the layer 2 (L2) chain alongside the opRollup system. This integration enables the seamless utilization of machine learning within smart contracts on the L2 chain. Based on this idea, we build an AI optimistic rollup layer 2 blockchain named ``Ls-a''.
``Ls-a'' enable users to seamlessly employ AI models natively within smart contracts without being encumbered by the intricacies of underlying technologies. By doing so, we aim to democratize access to AI-powered DApps, making AI model inferences both user-friendly and accessible.

Furthermore, with Ls-a and opML, we strive to deliver decentralized AI services that adhere to the core principles of blockchain technology, including trust, transparency, and security. By combining the strengths of blockchain and AI through opML, we envision a future where DApps can harness the full potential of AI models while preserving the ethos of decentralization and verifiable computation. This convergence opens doors to a new era of AI-powered smart contracts, offering a breadth of applications across various domains and industries.

% \subsection{Motivation}

% The integration of Artificial Intelligence (AI) with blockchain technology has opened new frontiers in the development of decentralized applications (DApps) with intelligent functionalities. However, a prevalent challenge in the current landscape of AI DApps is the infeasibility of conducting AI computations directly on-chain. Consequently, most of these applications resort to off-chain computations on centralized servers, only uploading the results onto the blockchain. While this approach may deliver results, it fundamentally lacks decentralization and gives rise to notable security concerns.

% % One alternative approach is to leverage Zero-Knowledge Machine Learning (ZKML), a privacy-focused solution that allows secure, verifiable computations. However, ZKML has its inherent limitations. Even when ZKML is used, it necessitates users to generate Zero-Knowledge Proofs (zk-proofs) for AI model inferences. This introduces complexity and additional steps, impeding the seamless and native utilization of AI models within smart contracts. Moreover, ZKML entails computational overhead, reducing its efficiency.

% In response to these challenges, we propose "Ls-a," an Optimistic Rollup Layer 2 (L2) blockchain integrated with opML (Optimistic Machine Learning on chain). Our motivation is to enable users to seamlessly employ AI models natively within smart contracts without being encumbered by the intricacies of underlying technologies. By doing so, we aim to democratize access to AI-powered DApps, making AI model inferences both user-friendly and accessible.

% Furthermore, with Ls-a and opML, we strive to deliver decentralized AI services that adhere to the core principles of blockchain technology, including trust, transparency, and security. By combining the strengths of blockchain and AI through opML, we envision a future where DApps can harness the full potential of AI models while preserving the ethos of decentralization and verifiable computation. This convergence opens doors to a new era of AI-powered smart contracts, offering a breadth of applications across various domains and industries.

\subsection{Overview}
% \subsection{Precompiled Contract Design}

Just like the existing rollup systems, ``Ls-a'' is responsible for "rolling up" transactions by batching them before publishing them to the L1 chain, usually through a network of sequencers. This mechanism could include thousands of transactions in a single rollup.
``Ls-a'' as one of the optimistic rollups, is an interactive scaling method for L1 blockchains. We optimistically assume that every proposed transaction is valid by default. Different from the traditional L2 optimistic rollup system, the transaction in ``Ls-a'' can include some AI model inferences, which can make the smart contracts on ``Ls-a'' ``smarter''.
In the case of mitigating potentially invalid transactions, like optimistic rollups, ``Ls-a'' introduces a challenge period during which participants may challenge a suspect rollup. A fraud-proving scheme is in place to allow for several fraud proofs to be submitted. Those proofs could make the rollup valid or invalid. During the challenge period, state changes may be disputed, resolved, or included if no challenge is presented (and the required proofs are in place).

To enable native AI inference in the smart contract, we need to modify the execution layer of the layer 2 chain. Specifically, we add a precompiled contract {\tt{inference}} in EVM. {\tt{inference}} will conduct the AI inference in native environment and then return deterministic execution results. As shown in Figure \ref{fig:example:AIcontract}, when a user wants to use the AI model to process some data, all he needs to to call the precompiled contract {\tt{inference}} with the model address and model input, and then he can obtain the model output and use it natively in the smart contract.

\begin{figure}[!h]
	\begin{footnotesize}
		\begin{lstlisting}[language=Solidity]
contract AIContract {
	...
	function model_inference(address model, bytes calldata input) public returns (bytes memory) {
        // inference is a precompiled contract
		bytes memory output = inference(model, input);
		return output;
	}
}
		\end{lstlisting}
	\end{footnotesize}
	\caption{An example of AI model inference in a contract.}
	\label{fig:example:AIcontract}
\end{figure}

The models are stored in the model data available (DA) layer. all the models can be retrieved from DA using the model address. 
% We add some precompiled models to the system for user convenience. As a future work, we will also allow the users to upload their own trained models to the model DA. The users need to pay for the model storage but can also obtain the reward from others using their provided models.
We assume the data availability of all the models. In the current implementation, we provide several precompiled models. As a future work, we will consider using an efficient DA layer for holding the models, and allow users to upload their own trained models to the DA. The users need to pay for the model storage but can also obtain the reward from others using their provided models.

% \todo{DA design? both for L1 and L2} 

% \todo{provide more details about how the AI inference is executed in the evm within the smart contract. Maybe we need to introduce the MLVM?}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/rollup.png}
%     \caption{System Architecture in AI Layer 2}
%     \label{fig:l2_arch}
% \end{figure}


\subsection{Workflow}

The sequence diagram of the workflow of ``Ls-a'' is shown in Figure \ref{fig:l2_sequence}.

\begin{figure}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/l2_sequence.png}
    \caption{Sequence Diagram in AI Layer 2}
    \label{fig:l2_sequence}
\end{figure}


\begin{enumerate}
    \item The basic workflow begins with users sending L2 transactions (we allow native AI inference in the smart contract) to a batcher node, usually the sequencer.
    \item Once the sequencer receives enough transactions, it will post them into an L1 smart contract as a batch.
    \item A validator node will read these transactions from the L1 smart contract and execute them on their local copy of the L2 state. As for the AI inference execution, the validator need to download model from model DA and conduct the AI inference within the opML engine.
    \item Once processed, a new L2 state is generated locally and the validator will post this new state root into an L1 smart contract. (Note that this validator can also be the sequencer.)
    \item Then, all other validators will process the same transactions on their local copies of the L2 state.
    \item They will compare their resultant L2 state root with the original one posted to the L1 smart contract.
    \item If one of the validators gets a different state root than the one posted to L1, they will begin a challenge on L1.
    \item The challenge will require the challenger and the validator that posted the original state root to take turns proving what the correct state root should be. This challenge process is also known as fraud proof. The fraud proof of ``Ls-a'' includes the fraud proof of L2 state transition and the fraud proof of opML.
    \item Whichever user loses the challenge, gets their initial deposit (stake) slashed. If the original L2 state root posted was invalid, it will be destroyed by future validators and will not be included in the L2 chain. 
\end{enumerate}


\subsection{Precompiled Contract}

The code design principle of the precompiled contract {\tt{inference}} is also following the design principles of opML, that is, we separate execution from proving. We provide two kinds of implementation of the precompiled contract {\tt{inference}}. One is compiled for native execution, which is optimized for high speed. Another is compiled for the fraud proof VM, which will help to prove the correctness of the opML results. 

As for the implementation for execution, we re-use the ML engine in opML. We will first fetch the model using the model address from the model hub and then load the model into the ML engine. ML engine will take the user's input in the precompiled contract as the model input and then execute the ML inference task. The ML engine can guarantee the consistency and determinism of the ML inference results using quantization and softloat (For more details, please refer to Section \ref{sec:consistency}). 

As for the implementation for proving, we introduce a special instruction {\tt{opML}}. This instruction takes the user's input and the model hash as the input, which are stored in the ``oracle key'' field in the FPVM memory space, and then returns opML result, which is stored in the  ``oracle value'' field in the FPVM memory space. This instruction is like an oracle. If you tell it the input of opML, it will return the result. Different from the ``hash oracle trick'' in the current optimistic rollup system such as Arbitrum \cite{kalodner2018arbitrum}, this oracle is like a computational oracle. And the correctness of this computational oracle is guaranteed by the fraud proof protocol.
% {We assume the data availability of all the models. In the current implementation, we provide several precompiled models. As a future work, we will consider using an efficient DA layer for holding the models, and allow users to upload their }

\subsection{Fraud Proof Design}

% In the fraud proof system of an optimistic rollup layer 2 chain ``Ls-a'', we need to cross-compile the modified {\tt{geth}} (the client of golang-ethereum on layer 2) to the fraud proof VM.


% We replace the precompiled contract {\tt{inference}} with a special fraud proof VM instruction {\tt{opML}}. Suppose it is the $k$-th executed instruction in the fraud proof VM. 

The core design principle of the fraud proof system of ``Ls-a'' is that we separate fraud proof process of {\tt{geth}} (the client of golang-ethereum on layer 2) and the opML.
Remind that we introduce a special instruction {\tt{opML}}, which can provide opML results for proving. Suppose it is the $k$-th instruction in the fraud proof VM execution trace.
As shown in Figure \ref{fig:l2_dispute}, in the dispute game, if the pinpointed step is the state $S_{i-1}$, where $i \neq k$. Then we just send (VM$_i$, S$_{i-1}$) to the onchain VM for arbitration. If the challenger produces a valid one-step proof, then he wins the challenge. Otherwise, the submitter wins the challenge.
If the pinpointed step is exactly state $S_{k-1}$, then we need to arbitrate the correctness of the opML result and we will go deep into the fraud proof protocol of opML. If the challenger provides a valid opML fraud proof, he wins the whole challenge. Otherwise, the submitter wins the challenge.

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/l2_dispute.png}
    \caption{Dispute Game in ``Ls-a''}
    \label{fig:l2_dispute}
\end{figure}

We now focus on the special scenario, where the pinpointed step is exactly state $S_{i-1}, (i = k)$, and we need to go deep into the fraud proof protocol of opML.
% To prove the correctness of the entrance to the opML fraud proof, we need to prove the correctness of the construction of the initial FPVM state in opML. 
For convenience, we denote the initial FPVM state in opML as $M_0$ (Both the challenger and submitter share the same initial state). The submitter's final FPVM state in opML is denoted as $M_m$, and the challenger's final FPVM state in opML is denoted as $M'_m$. As shown in Figure \ref{fig:l2_dispute}, both the submitter and challenger agree on the $(i-1)$-th L2 state, i.e., $S_{i-1} = S'_{i-1}$, but disagree with the next state, i.e., $S_{i} \neq S'_{i}$. In this case, we need to go deep into the fraud proof protocol of opML for further arbitration. To guarantee the correctness and safety of the fraud proof protocol, we need to check the correctness and consistency of the state transition:
\begin{enumerate}
    \item \textit{Correctness of the entrance to opML}. We need to prove the correctness of the construction of the initial FPVM state in opML $M_0$ from L2 state $S_{i-1}$, that is, $S_{i-1} \Leftrightarrow M_0$
    \item \textit{Consistency of the exit of opML}. We need to check the consistency of the final state in opML and the layer 2 dispute state, i.e., $S_i \Leftrightarrow M_m \land S'_i \Leftrightarrow M'_m$.
\end{enumerate}

As shown in Figure \ref{fig:l2_transition}, the memory of the fraud proof VM (FPVM) is organized as a Merkle tree.  To prove (1) the correctness of the entrance to opML and (2) the consistency of the exit of opML, we can prove by using the Merkle proof and the reconstruction of the Merkle tree.

\begin{figure}
    \centering
    \includegraphics[width=0.98\textwidth]{figures/L2_opml.pdf}
    \caption{State Transition between Layer 2 and opML}
    \label{fig:l2_transition} 
\end{figure}


\begin{algorithm}
\SetKw{}{}
% \SetAlgoNlRelativeSize{0}
% \SetNlSty{textbf}{(}{)}
% \SetAlgoNlRelativeSize{0}
\SetNlSty{textbf}{\{}{\}}
\DontPrintSemicolon
\LinesNumbered
\KwIn{(1) Layer 2 state root $S_{i-1}$, (2) opML FPVM memory root $M_0$, (3) Merkle subtree root of ``oracle key'' field $r_k$ in Layer 2 state, (4) Merkle proof $p_k$ of $r_k$} %, (5) Merkle subtree root $r_i$ in opML state, (6) Merkle proof $p_i$ of $r_i$
% \KwOut{True or False}
\SetKwFunction{ConstructMerkleTree}{ConstructMerkleTree}
\SetKwFunction{MerkleCheck}{MerkleCheck}
\SetKwFunction{FMain}{EntranceCorrectnessCheck}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FMain{$S_i, M_0, r_k, p_k$}}{
    $A_k  \longleftarrow $ memory address of ``oracle key'' in FPVM; \;
    \textbf{require} \MerkleCheck{$S_{i-1}$, $r_k$, $p_k$ $A_k$} \;
    $A_p  \longleftarrow $ memory address of ``opML program'' in FPVM; \;
    $A_m  \longleftarrow $ memory address of ``model'' in FPVM; \;
    $A_i  \longleftarrow $ memory address of ``input'' in FPVM; \;
    $r_p \longleftarrow $ Merkle subtree root of ``opML program'' \;
    $r_m \longleftarrow $ Merkle subtree root of ``model'' \;
    $r_i \longleftarrow r_k$ (Merkle subtree root of ``input'') \;
    $M^*_0 \longleftarrow $ \ConstructMerkleTree{$r_p$, $A_p$, $r_i$, $A_i$, $r_m$, $A_m$} \;
    \textbf{require} $M^*_0 == M_0$ \;
    \textbf{return} True \; 
}
\caption{Correctness of the Entrance to opML}
\label{algo:entrance}
\end{algorithm}

To guarantee the  correctness of the entrance to opML, we need to correctly construct the Merkle tree of the initial FPVM state in opML, which is shown in Algorithm \ref{algo:entrance}.
As shown in Figure \ref{fig:l2_transition}, we need to construct the Merkle tree of the opML state memory as follows. The opML program and the model are public known. The ``input'' field in the opML FPVM memory is consistent with the ``oracle key'' field in the L2 FPVM memory. The ``output'' field of opML FPVM memory is empty at the initial state, and will be filled in the after the opML execution. The ``oracle key'' and the ``oracle value'' field are also empty at the initial state. With these fields, we can construct the initial FPVM state in opML. 
Due to complexity and gas limitations, we would not run Algorithm \ref{algo:entrance} in the smart contract on chain. Instead, we build a zero-knowledge circuit to check the correctness of the entrance to opML and verify the zero-knowledge proof on chain.



\begin{algorithm}
\SetKw{}{}
% \SetAlgoNlRelativeSize{0}
% \SetNlSty{textbf}{(}{)}
% \SetAlgoNlRelativeSize{0}
\SetNlSty{textbf}{\{}{\}}
\DontPrintSemicolon
\LinesNumbered
\KwIn{(1) Layer 2 state root $S_i$, (2) opML FPVM memory root $M_m$, (3) Merkle subtree root $r_o$ of ``output'' field in opML state, (4) Merkle proof $p_o$ of $r_o$, (5) Merkle subtree root $r_v$ of ``oracle value'' field in L2 state, (6) Merkle proof $p_v$ of $r_v$}    
% \KwOut{True or False}
\SetKwFunction{MerkleCheck}{MerkleCheck}
\SetKwFunction{FMain}{ExitConsistencyCheck}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FMain{$S_i, M_m, r_0, p_o, r_v, p_v$}}{
    $A_o  \longleftarrow $ memory address of ``output'' in FPVM; \;
    $A_v  \longleftarrow $ memory address of ``oracle value'' in FPVM; \;
    \textbf{require} \MerkleCheck{$S_i$, $r_v$, $p_v$ $A_v$} \;
    \textbf{require} \MerkleCheck{$M_m$, $r_o$, $p_o$, $A_o$} \;
    \textbf{require} $r_o == r_v$ \;
    \textbf{return} True \; 
}
\caption{Consistency of the Exit of opML}
\label{algo:exit}
\end{algorithm}

Algorithm \ref{algo:exit} shows the algorithm to check the consistency of the exit of opML.
To prove the consistency of the exit of opML, we need to prove that the Merkle subtree root of ``output'' field $r_o$ in opML FPVM memory  is consistent with the Merkle subtree root of the ``oracle value'' field $r_v$ in layer 2 FPVM memory. That is, to check the consistency of $S_i \Leftrightarrow M_m$, we provide a Merkle proof of the subtree root $r_o$ in the Merkle tree with root $M_m$ and the Merkle proof of the subtree root $r_v$ in the Merkle tree with root $S_i$, and then check $r_o = r_v$.  

==> optimization.tex <==
\section{Optimization}

Furthermore, we can utilize multiple checkpoints and multi-step ZK verifier to provide a zk-fraud proof to speed up the finality of opML. Assuming that there are $N$ steps in the opML fraud proof VM. Then the number of interactions would be $O(\log_2(N))$. One optimization approach to reduce to the interactions is to use a multi-step on-chain arbitrator, instead of only one-step on-chain arbitrator.

This can be done by using a zkVM, e.g., zkWASM, RICS Zero, Cairo VM, which can provide zk-proof for the multi-step execution. Suppose the zkVM can generate a zk-proof for $m$ steps, then the number of interactions can be reduce from $O(\log_2(N))$ to $O(\log_2(N/m))$. Besides, instead of using bisection protocol with only 1 checkpoint, we can provide multiple checkpoints (for example $k$ ($k >1$) checkpoints) in the dispute game (verification game). At this time, we can further reduce the interactions number from $O (\log_2(N/m))$ to $O( \log_{k+1}(N/m))$. With these optimizations, we can greatly speed up the finality of opML, and it is possible to achieve almost instant confirmation!

==> privacy.tex <==
\section{OPPA: Privacy-Preserving opML}\label{sec:privacy}



==> single-phase.tex <==
\section{Single-Phase Dispute Game}

The one-phase pinpoint protocol works similarly to referred delegation of computation (RDoC), where two or more parties (with at least one honest party) are assumed to execute the same program. Then, the parties can challenge each other with a pinpoint style to locate the disputable step. The step is sent to a judge with weak computation power (smart contract on blockchain) for arbitration. 

In one-phase opML:

\begin{itemize}
    \item We build a virtual machine (VM) for offchain execution and onchain arbitration. We guarantee the equivalence of the offchain VM and the onchain VM implemented on a smart contract.
    \item To ensure the efficiency of AI model inference in the VM, we have implemented a lightweight DNN library specifically designed for this purpose instead of relying on popular ML frameworks like Tensorflow or PyTorch. Additionally, a script that can convert Tensorflow and PyTorch models to this lightweight library is provided.
    \item The cross-compilation technology has been applied to compile the AI model inference code into the VM program instructions.
    \item The VM image is managed with a Merkle tree, only the Merkle root will be uploaded to the onchain smart contract. (The Merkle root stands for the VM state.)
    \item The bisection protocol will help to locate the dispute step, the step will be sent to the arbitration contract on the blockchain
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/image.png}
    \caption{Sequence Diagram in AI Layer 2}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/dispute.png}
    \caption{Sequence Diagram in AI Layer 2}
    \label{fig:enter-label}
\end{figure}
